Model-agnostic Feature Importance and Effects with Dependent Features -- A Conditional Subgroup Approach

The interpretation of feature importance in machine learning models is challenging when features are dependent. Permutation feature importance (PFI) ignores such dependencies, which can cause misleading interpretations due to extrapolation. A possible remedy is more advanced conditional PFI approaches that enable the assessment of feature importance conditional on all other features. Due to this shift in perspective and in order to enable correct interpretations, it is therefore important that the conditioning is transparent and humanly comprehensible. In this paper, we propose a new sampling mechanism for the conditional distribution based on permutations in conditional subgroups. As these subgroups are constructed using decision trees (transformation trees), the conditioning becomes inherently interpretable. This not only provides a simple and effective estimator of conditional PFI, but also local PFI estimates within the subgroups. In addition, we apply the conditional subgroups approach to partial dependence plots (PDP), a popular method for describing feature effects that can also suffer from extrapolation when features are dependent and interactions are present in the model. We show that PFI and PDP based on conditional subgroups often outperform methods such as conditional PFI based on knockoffs, or accumulated local effect plots. Furthermore, our approach allows for a more fine-grained interpretation of feature effects and importance within the conditional subgroups.

==> figures/data-fidelity.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Sat Mar 28 05:16:40 2020
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrrrrrrrrrrrrr}
  \hline
 & space\_ga\_KNN(k=7) & space\_ga\_Linear Model & space\_ga\_Random Forest & wind\_KNN(k=7) & wind\_Linear Model & wind\_Random Forest & satellite\_image\_KNN(k=7) & satellite\_image\_Linear Model & satellite\_image\_Random Forest & pollen\_KNN(k=7) & pollen\_Linear Model & pollen\_Random Forest & wine\_quality\_KNN(k=7) & wine\_quality\_Linear Model & wine\_quality\_Random Forest & quake\_KNN(k=7) & quake\_Linear Model & quake\_Random Forest \\ 
  \hline
1 & 0.04 & 0.04 & 0.16 & 45.16 & 43.01 & 46.04 & 4.71 & 4.79 & 4.80 & 9.76 & 9.86 & 9.86 & 0.72 & 0.73 & 0.74 & 0.04 & 0.04 & 0.04 \\ 
  2 & 0.04 & 0.03 & 0.16 & 45.15 & 42.80 & 46.06 & 4.70 & 4.81 & 4.80 & 9.71 & 9.75 & 9.86 & 0.72 & 0.73 & 0.74 & 0.04 & 0.04 & 0.04 \\ 
  3 & 0.03 & 0.03 & 0.12 & 29.05 & 28.25 & 29.87 & 4.38 & 4.56 & 4.46 & 8.42 & 9.13 & 9.48 & 0.69 & 0.71 & 0.70 & 0.04 & 0.04 & 0.04 \\ 
  4 & 0.03 & 0.02 & 0.02 & 18.15 & 18.38 & 18.23 & 1.94 & 2.15 & 2.45 & 6.75 & 7.20 & 6.45 & 0.56 & 0.59 & 0.61 & 0.04 & 0.04 & 0.04 \\ 
  5 & 0.03 & 0.03 & 0.10 & 24.97 & 25.24 & 26.31 & 3.20 & 3.16 & 3.22 & 8.10 & 8.72 & 8.26 & 0.68 & 0.69 & 0.70 & 0.04 & 0.04 & 0.04 \\ 
  6 & 0.03 & 0.03 & 0.03 & 19.66 & 19.79 & 19.62 & 2.50 & 2.59 & 2.85 & 6.92 & 7.36 & 6.53 & 0.61 & 0.63 & 0.63 & 0.04 & 0.04 & 0.04 \\ 
   \hline
\end{tabular}
\caption{Median model fidelity over the features} 
\label{tab:model-fidelity}
\end{table}


==> latex-math/chapter-notation.tex <==
\section{General Notation and Terminology}
\label{sec:notation}

Consider a $p-$dimensional feature space $\Xspace = (\Xspace[1] \times \Xspace[2] \times \hdots \times \Xspace[p])$ %of arbitrary measurement scales
and a target space $\Yspace$.
Suppose that there is an unknown functional relationship $f$ between $\Xspace$ and $\Yspace$.
ML algorithms try to learn this relationship using training data with observations that have been drawn i.i.d. from an unknown probability distribution $\mathcal{P}$ on the joint space $\Xspace \times \Yspace$.
%The learned prediction model will be denoted by $\fh$ and approximates $f$.
We consider an arbitrary prediction model $\fh$, fitted on some training data to approximate $f$ and analyze it with model-agnostic interpretability methods.
Let $\D = \Dset$ be a test data set sampled i.i.d. from $\mathcal{P}$ where $n$ is the number of observations in the test set.
Let $P = \{1, \hdots, p\}$ be an index set referring to all features.
We denote the corresponding random variables generated from the feature space by $X = (X_1, \hdots, X_p)$ and the random variable generated from the target space by $Y$.
In our notation, the vector $\xi = \xivec \in \Xspace$ refers to the $i$-th observation which is associated with the target outcome $\yi \in \Yspace$ and $\xj = \xjvec$ denotes the realizations of the $j$-th feature.
%Suppose that there is an unknown functional relationship $f$ that maps each observation $\xi$ to its target outcome $\yi$.
% Performane estimation
% The performance estimation of a ML algorithm is based on training the algorithm on training data and estimating the \emph{generalization error} (also known as \emph{test error}) of the algorithm on new (unseen) test data.
We denote the generalization error of a fitted model on unseen test data from $\mathcal{P}$ by $GE(\fh, \mathcal{P}) = \E(L(\fh(X), Y))$, measured by a loss function $L$.
%with which the performance of $\fhD$ is measured.
It can be estimated using the test data $\D$ by %through the empirical expected loss
%by splitting the observed data $\D$ into a training set $\Dtrain$ and test set $\Dtest = \D \setminus \Dtrain$, fitting the model on the training set and averaging the loss or gain function over an independent test set using
\begin{equation}
\label{eq:geest}
%\GEh{}(\fh, \D) = \frac{1}{|\D|} \sum_{\xy \in \D} L(\fh(x), y).
\textstyle \GEh{}(\fh, \D) = \frac 1 n \sum_{i=1}^n \Lii.
\end{equation}
%Note that if $\fh$ was trained on $\D$ and if the generalization error uses again $\D$ to measure the performance, we obtain an estimate for the training error.
%We therefore consider $\fh$ as a fixed model that was trained on $\Dtrain$ which is i.i.d. from $\D$. %the observations from the data set $\D$ were not used to fit the model $\fh$.
A better estimate for the generalization error of an ML algorithm can be obtained using resampling techniques such as cross-validation or bootstrap \citep{Bischl2012}. %as they %reuse the observed data at hand to produce a better estimator.
%Specifically, they repeatedly split the observed data into training and test sets of equal size, fit a model using the produced training sets and estimate the performance on the remaining test sets.
%The resulting performance values on each test set are then aggregated by averaging in order to estimate the generalization error more precisely \citep[see e.g.][]{Bischl2012}.


==> latex-math/ml-bagging.tex <==
% ml - bagging, random forest

\newcommand{\bl}[1]{b^{[#1]}(x)}											% baselearner with argument for m
\newcommand{\blm}{\bl{m}}												    % baselearner without argument for m
\newcommand{\blmh}{\hat{b}^{[m]}(x)}										% estimated base learner 
\newcommand{\fM}{f^{[M]}(x)}                    % ensembled predictor


==> latex-math/ml-boosting.tex <==
% ml - boosting
\newcommand{\fm}{f^{[m]}}                                                   % prediction in iteration m
\newcommand{\fmh}{\hat{f}^{[m]}}                                            % prediction in iteration m
\newcommand{\fmd}{f^{[m-1]}}                                                % prediction m-1
\newcommand{\fmdh}{\hat{f}^{[m-1]}}                                         % prediction m-1
\newcommand{\bmm}{b^{[m]}}                                                  % basemodel m
\newcommand{\bmmh}{\hat{b}^{[m]}}                                           % basemodel m with hat
\newcommand{\betam}{\beta^{[m]}}                                            % weight of basemodel m
\newcommand{\betamh}{\hat{\beta}^{[m]}}                                     % weight of basemodel m with hat
\newcommand{\betai}[1]{\beta^{[#1]}}                                        % weight of basemodel with argument for m
\newcommand{\errm}{\text{err}^{[m]}}                                        % weighted in-sample misclassification rate
\newcommand{\wm}{w^{[m]}}                                                   % weight vector of basemodel m
\newcommand{\wmi}{w^{[m](i)}}                                               % weight of obs i of basemodel m
\newcommand{\thetam}{\theta^{[m]}}                                          % parameters of basemodel m
\newcommand{\thetamh}{\hat{\theta}^{[m]}}                                   % parameters of basemodel m with hat
\newcommand{\rmm}{r^{[m]}}                                                  % pseudo residuals
\newcommand{\rmi}{r^{[m](i)}}                                               % pseudo residuals
\newcommand{\Rtm}{R_{t}^{[m]}}                                              % terminal-region
\newcommand{\Tm}{T^{[m]}}                                                   %
\newcommand{\ctm}{c_t^{[m]}}                                                % mean, terminal-regions
\newcommand{\ctmh}{\hat{c}_t^{[m]}}                                         % mean, terminal-regions with hat
\newcommand{\ctmt}{\tilde{c}_t^{[m]}}                                       % mean, terminal-regions
\newcommand{\fxk}{f_k(x)}                                                   % f_k(x)
\newcommand{\Lp}{L^\prime}
\newcommand{\Ldp}{L^{\prime\prime}}
\newcommand{\Lpleft}{\Lp_{\text{left}}}

==> latex-math/ml-gp.tex <==
% ml - Gaussian Process

\newcommand{\gp}{\mathcal{GP}\left(m(x), k\left(x, x'\right)\right)} 								% Gaussian Process Definition	
\newcommand{\mvec}{\bm{m}}												    						% Gaussian process mean vector
\newcommand{\Kmat}{\bm{K}}																			% estimated base learner 
\newcommand{\ls}{\ell}                                           % length-scale


==> latex-math/ml-mbo.tex <==
% ml - MBO
\newcommand{\sxh}{\hat{s}(x)} % uncertainty shat(x)
\newcommand{\vxh}{\hat{s}^2(x)}
\newcommand{\matK}{\mathbf{K}}
\newcommand{\kstarx}{\mathbf{k}_*(x)}
\newcommand{\xpi}[1][i]{x^{*(#1)}}
\newcommand{\vhx}{\ensuremath{\sh^2(\xv)}\xspace}          % local estimated variance at point x
\newcommand{\shx}{\ensuremath{\sh(\xv)}\xspace}            % local estimated uncertainty at point x
\newcommand{\sh}{\ensuremath{\hat{s}}\xspace}              % local estimated uncertainty
\newcommand{\px}{\ensuremath{\boldsymbol{x}^*}}
\newcommand{\equote}[1]{``#1''}
\newcommand{\vecx}{\ensuremath{\boldsymbol{x}}}
\newcommand{\yx}{\ensuremath{y(\vecx)}}
\newcommand{\X}{\ensuremath{\mathcal{X}}\xspace}           % domain / search space

% already defined in basic-math:
% \newcommand{\yv}{\boldsymbol{y}}
\newcommand{\fhx}{\ensuremath{\fh(\xv)}\xspace}            % surrogate (x), better use \mhx for predicted value

==> latex-math/ml-nn.tex <==
% ml - NNs
\newcommand{\neurons}{z_1,\dots,z_M} % vector of neurons

\newcommand{\hidz}{\mathbf{z}}                            % vector of hidden activations
\newcommand{\biasb}{\mathbf{b}}                           % bias vector
\newcommand{\wtw}{\mathbf{w}}                             % weight vector (general)
\newcommand{\wtu}{\mathbf{u}}                             % weight vector of output neuron
%


% deeplearning - regularization
\newcommand{\Oreg}{\mathnormal{R}_{reg}(\theta|X,y)}				% regularized objective function
\newcommand{\Ounreg}{\mathnormal{R}_{emp}(\theta|X,y)}			% unconstrained objective function
\newcommand{\Pen}{\Omega(\theta)}							% penalty
\newcommand{\Oregweight}{\mathnormal{R}_{reg}(w|X,y)}			% regularized objective function with weight 
\newcommand{\Oweight}{\mathnormal{R}_{emp}(w|X,y)}				% unconstrained objective function with weight
\newcommand{\Oweighti}{\mathnormal{R}_{emp}(w_i|X,y)}			% unconstrained objective function with weight w_i
\newcommand{\Oweightopt}{\mathnormal{J}(w^*|X,y)}				% unconstrained objective function withoptimal  weight
\newcommand{\Oopt}{\hat{\mathnormal{J}}(\theta|X,y)}				% optimal objective function 
\newcommand{\Odropout}{\mathnormal{J}(\theta, \mu|X,y)}	           	% dropout objective function

% deeplearning - optimization
\newcommand{\Lmomentum}{L(\yi, f(x^{(i)}, \theta + \varphi \nu))}                  % momentum risk

% deeplearning - autoencoders
\newcommand{\uauto}{L(x,g(f(x)))}			% undercomplete autoencoder objective function
\newcommand{\dauto}{L(x,g(f(\tilde{x})))}		% denoising autoencoder objective function


==> latex-math/ml-svm.tex <==
% ml - svms
\newcommand{\sv}{\operatorname{SV}}                                         % supportvectors
% already defined in basic-math:
% \newcommand{\HS}{\mathcal{H}}                                               % H, hilbertspace
\renewcommand{\sl}{\zeta}
\newcommand{\slvec}{\left(\zeta^{(1)}, \zeta^{(n)}\right)}		% slack variables (SVM)
\newcommand{\sli}{\zeta^{(i)}}																% slack variable (SVM)


==> latex-math/ml-trees.tex <==
% ml - trees, extra trees

\newcommand{\Np}{\mathcal{N}}												% (Parent) node N
\newcommand{\Nl}{\Np_1}														% Left node N_1
\newcommand{\Nr}{\Np_2}														% Right node N_2
\newcommand{\pikN}{\hat{\pi}_{\Np k}}             % estimated class probability in N

